What Happens Next? Anticipating Future Motion by Generating Point Trajectories

We consider the problem of forecasting motion from a single image, i.e., predicting how objects in the world are likely to move, without the ability to observe other parameters such as the object velocities or the forces applied to them. We formulate this task as conditional generation of dense trajectory grids with a model that closely follows the architecture of modern video generators but outputs motion trajectories instead of pixels. This approach captures scene-wide dynamics and uncertainty, yielding more accurate and diverse predictions than prior regressors and generators. We extensively evaluate our method on simulated data, demonstrate its effectiveness on downstream applications such as robotics, and show promising accuracy on real-world intuitive physics datasets. Although recent state-of-the-art video generators are often regarded as world models, we show that they struggle with forecasting motion from a single image, even in simple physical scenarios such as falling blocks or mechanical object interactions, despite fine-tuning on such data. We show that this limitation arises from the overhead of generating pixels rather than directly modeling motion.

==> sections/06_equations.tex <==
\[
\mathcal{L}_\text{RF}( \theta)
=
\mathbb{E}_{\vec{z}_0,(\vec{z}_1,\Image),t}
\left[
    \|
    \hat \bv_\theta((1-t) \vec{z}_0 + t \vec{z}_1, t, \Image) - (\vec{z}_1 - \vec{z}_0)
    \|^2_2 
\right], \quad \vec{z}_0 \sim \mathcal{N}_0
\]

\[
\mathcal{L}_{\beta\text{-VAE}}(\enc, \dec, \vec{x}, \Image)
=
\mathbb{E}_{\vec{z} \sim \mathcal{N}_{\enc(\vec{x} \mid \Image)}}
\left[
    \underbrace{L_{\delta}\left(
        \vec{x}, \dec(\vec{z} \mid \Image)
    \right)}_{\text{Huber Loss}}
\right]
+
\beta \cdot \mathbb{D}_{\mathrm{KL}}
\left(
    \mathcal{N}_{\enc(\vec{x} \mid \Image)} \parallel
    \mathcal{N}_0
\right)
\]

\[
\vec{z}_1 - \vec{z}_0 = \int_{0}^{1} \hat{\bv}_\theta(\vec{z}_t, t, \Image) \, \mathrm{d}t
\]

\begin{table}[ht]
    \centering
    \begin{tabular}{llcccc}
        \toprule
        \textbf{Latent Space} & \textbf{Latent Shape} & \textbf{FVMD} & \textbf{FVMD (S)} & \textbf{Best-Of-K} & \textbf{LRTL} \\
        \midrule
        \multicolumn{6}{l}{\textit{Kubric (In-Distribution)}} \\
        SD3.5          & 24$\times$16$\times$16$\times$16 & 16592 & 21869 & 147 & 33.7 \\
        SD3.5 + Tracks & 24$\times$24$\times$16$\times$16 & \underline{15399} & \underline{20414} & \underline{136} & \underline{28.2} \\
        \textbf{Tracks} & 24$\times$16$\times$16$\times$8 & \textbf{12221} & \textbf{14950} & \textbf{127} & \textbf{15.9} \\
        \midrule
        \multicolumn{6}{l}{\textit{Kubric (Out-Of-Distribution)}} \\
        SD3.5          & 24$\times$16$\times$16$\times$16 & 13661 & 17004 & \underline{115} & 28.0 \\
        SD3.5 + Tracks & 24$\times$24$\times$16$\times$16 & \underline{13386} & \underline{16694} & \textbf{109} & \underline{24.6} \\
        \textbf{Tracks} & 24$\times$16$\times$16$\times$8 & \textbf{12062} & \textbf{14748} & 129 & \textbf{18.4} \\
        \bottomrule
    \end{tabular}
    \vspace{5pt} % Optional: adds a bit of space before the caption
    \caption{Performance comparison across different latent spaces.}
    \label{tab:latent_comparison}
\end{table}

==> sections/A_acknowledgements.tex <==
\section*{Acknowledgements}
We thank Jensen (Jinghao) Zhou for sharing his insights on training stability in diffusion models. We are also grateful to Ruining Li, Stan Szymanowicz, Lorenza Prospero, Zihang Lai, Zeren Jiang, and Minghao Chen for their helpful suggestions.

==> sections/A_metrics.tex <==

\subsection{Assessing metrics}

We investigate the validity of our distributional metrics in \cref{tab:metric_check}.
Here, we make use of our Kubric evaluation set, but we partition it into two sets, such that each scene has 32 possible futures.
Intuitively, ground truth data should be a very good predictor of itself.
We compare the values against simply running CoTracker to predict the motion of points on the ground truth video.
All metrics are lower when ground truth is used to predict ground truth.
\input{tables/metric_sanity}


==> sections/rest.tex <==

\clearpage
%---especially given the modest size of our model and training data (about 5,000 synthetic videos). %\GB{Somehow connect this to abstract point trajectories and hypothesize they should generalize better than pixels. Perhaps include samples from SoTa physical generators on these two examples.}

\input{tables/time_memory}

\paragraph{Efficiency.}
%\GB{This is not an apples-to-apples comparison. However, both are latent, and we use a latent code of the same dimension as the video generators. Thus, it is a reasonable comparison. In addition, dense trajectory extraction is rarely required for other tasks. Point trackers are still too slow for this. \textbf{Say that diffusing tracks is simply faster than the pipeline (video + cotrack)} }
In \cref{tab:time_memory}, we compare the time and memory required to sample a $32 \times 32$ grid from our model. Modelling trajectories is significantly more efficient (i.e., several orders of magnitude) than modelling pixels in terms of wall-clock time, GPU memory usage, and parameter count.
This efficiency largely stems from our trajectory denoiser being much smaller than the denoisers used for video generation.

%\todo{Show a figure where we sample a trajectory in a few steps.}



\paragraph{Limitations.}

We discuss the limitations of our method in the supplementary material, including the challenge of learning from real data, which is an advantage of video generators.



==> tables/vae.tex <==
\begin{table}[htb]
\centering
\small
\caption{
\textbf{Our VAE configuration}.
}
    \label{tab:denoiserconfigs} % Added a label for referencing
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Model} & \textbf{Number of Encoder Autoencoding Blocks} & \textbf{Number of Decoder Autoencoding Blocks}  & \textbf{Hidden size} & \textbf{Heads} & \textbf{Parameter Count (M)} \\
    \midrule
    \textbf{Base (B)}  & 6 & 6 & 384 & 6 & 41.7 \\
    \bottomrule
    \end{tabular}
\end{table}
